Low-Complexity Block-Based Decoding Algorithms for Short Block Channels

This paper presents low-complexity block-based encoding and decoding algorithms for short block length channels. In terms of the precise use-case, we are primarily concerned with the baseline 3GPP Short block transmissions in which payloads are encoded by Reed-Muller codes and paired with orthogonal DMRS. In contemporary communication systems, the short block decoding often employs the utilization of DMRS-based least squares channel estimation, followed by maximum likelihood decoding. However, this methodology can incur substantial computational complexity when processing long bit length codes. We propose an innovative approach to tackle this challenge by introducing the principle of block/segment encoding using First-Order RM Codes which is amenable to low-cost decoding through block-based fast Hadamard transforms. The Block-based FHT has demonstrated to be cost-efficient with regards to decoding time, as it evolves from quadric to quasi-linear complexity with a manageable decline in performance. Additionally, by incorporating an adaptive DMRS/data power adjustment technique, we can bridge/reduce the performance gap and attain high sensitivity, leading to a good trade-off between performance and complexity to efficiently handle small payloads.

==> figures/tikz/ray/comp_optim_tdl.tex <==

% \pgfplotsset{
%     tick label style={font=\footnotesize},
%     label style={font=\footnotesize},
%     legend style={nodes={scale=0.7, transform shape}, font=\tiny, legend cell align=left},
%     every axis/.append style={line width=0.5pt}
% }



%legend pos=outer north east
%legend pos=north west
%legend pos=north east
\pgfplotsset{
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    legend style={nodes={scale=0.55, transform shape}, font=\tiny, legend cell align=left},
    every axis/.append style={line width=0.5pt}
}

%legend pos=outer north east
%legend pos=north west
%legend pos=north east

      \begin{tikzpicture}
              \begin{semilogyaxis}[xlabel=SNR (dB),
            ,ylabel=BLER,
            %legend pos=south west,
            legend columns=2,
            legend style={at={(0.5,1.02)},anchor=south},
            grid=both, xmin=-10,xmax=4, ymin=0.001,ymax=0.3]



\addplot+[smooth,teal, dotted, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
(-4,	0.1454)
(-3,	0.0726)
(-2,	0.0277)
(-1,	0.0094)
(0, 0.0024)
(1, 0.0003)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=2}

\addplot+[smooth,teal, dashed, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
(-6,	0.1123)
(-5,	0.0438)
(-4,	0.0161)
(-3,	0.0035)
(-2,	0.0008)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=4}


\addplot+[smooth,teal, solid, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
%(-9,	0.175)
%(-9,	0.2192)
(-8,	0.0959)
(-7, 0.0293)
(-6, 	0.0082)
(-5, 	0.001)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=8}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%deja bon%%%%%%%%%%
\addplot+[smooth, dotted, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
%(-3,	0.1898)
(-2,	0.0998)
(-1,	0.0549)
(0,	0.022)
(1,	0.0072)
(2,	0.0019)
(3,	0.0007)
(4,	0.0001)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=2}

\addplot+[smooth, dashed, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
%(-6,	0.243)
(-5,	0.1449)
(-4,	0.072)
(-3,	0.0294)
(-2,	0.0102)
(-1,	0.0029)
(0,	0.0003)
(1,	0.0002)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=4}

\addplot+[smooth, solid, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
%(-8,	0.2196)
(-7,	0.1178)
(-6,	0.057)
(-5,	0.0196)
(-4,	0.0031)
(-3,	0.0003)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=8}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot+[smooth, dotted, olive, mark options={ scale=1, fill=olive, solid},mark=otimes] coordinates {
(-3, 	0.1898)
(-2, 	0.0998)
(-1, 	0.0549)
(0	, 0.022)
(1	, 0.0072)
(2	, 0.0019)
(3	, 0.0007)
(4	, 0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2}


\addplot+[smooth, dashed, olive, mark options={ scale=1, fill=olive, solid },mark=otimes] coordinates {
(-5, 	0.1449)
(-4, 	0.072)
(-3, 	0.0294)
(-2, 	0.0102)
(-1, 	0.0029)
(0	, 0.0003)
(1	, 0.0002)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4}

\addplot+[smooth, solid, olive, mark options={ scale=1, fill=olive},mark=otimes] coordinates {
(-7, 	0.1178)
(-6, 	0.057)
(-5, 	0.0196)
(-4, 	0.0031)
(-3, 	0.0003)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot+[smooth,orange, dotted, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-3, 	0.1633)
(-2, 	0.0837)
(-1, 	0.0436)
(0	, 0.0186)
(1	, 0.0054)
(2	, 0.0011)
(3	, 0.0005)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2, $\beta = 1.25$}

\addplot+[smooth,orange, dashed, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-5, 	0.1133)
(-4, 	0.0512)
(-3, 	0.0198)
(-2, 	0.0063)
(-1, 	0.0013)
(0	, 0.0003)
(1	, 0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4, $\beta = 1.25$}

\addplot+[smooth,orange, solid, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-8, 	0.1615)
(-7, 	0.0802)
(-6, 	0.0338)
(-5, 	0.0113)
(-4, 	0.002)
(-3, 	0.0001)

};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8, $\beta = 1.25$}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot+[smooth,green, dotted, mark options={scale=1, fill=green, solid},mark=]coordinates {
(-3, 	0.1473)
(-2, 	0.0762)
(-1, 	0.0402)
(0	, 0.0157)
(1	, 0.0049)
(2	, 0.0013)
(3	, 0.0005)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2, $\beta = 1.50$}


\addplot+[smooth,green, dashed, mark options={scale=1, fill=green, solid},mark=]coordinates {
%(-6, 	0.1851)
(-6, 	0.1663)
(-5, 	0.0982)
(-4, 	0.043)
(-3, 	0.0156)
(-2, 	0.0054)
(-1, 	0.0011)
(0	, 0.0002)
(1	, 0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4, $\beta = 1.50$}

\addplot+[smooth,green, solid, mark options={scale=1, fill=green, solid},mark=]coordinates {
(-8, 	0.1278)
(-7, 	0.0601)
(-6, 	0.0251)
(-5, 	0.0067)
(-4, 	0.0014)
(-3, 	0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8, $\beta = 1.50$}
%
%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\addplot+[smooth,cyan, dotted, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
%-7	0.2666)
(-3, 	0.1388)
(-2, 	0.07)
(-1, 	0.0378)
(0	, 0.0143)
(1	, 0.0043)
(2	, 0.0013)
(3	, 0.0003)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2, $\beta = 1.75$}
%
\addplot+[smooth,cyan, dashed, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
%-7	0.2666)
(-6, 	0.1517)
(-5, 	0.0873)
(-4, 	0.0385)
(-3, 	0.0135)
(-2, 	0.0044)
(-1, 	0.001)
(0	, 0.0001)
(1	, 0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4, $\beta = 1.75$}
%
%
\addplot+[smooth,cyan, solid, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
(-8, 	0.1121)
(-7, 	0.0488)
(-6, 	0.0194)
(-5, 	0.0055)
(-4, 	0.001)
(-3, 	0)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8, $\beta = 1.75$}

%%%%%%%
        \end{semilogyaxis}
    \end{tikzpicture}


==> figures/tikz/ray/comp_optim_tdl_scalled.tex <==

% \pgfplotsset{
%     tick label style={font=\footnotesize},
%     label style={font=\footnotesize},
%     legend style={nodes={scale=0.7, transform shape}, font=\tiny, legend cell align=left},
%     every axis/.append style={line width=0.5pt}
% }



%legend pos=outer north east
%legend pos=north west
%legend pos=north east
\pgfplotsset{
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    legend style={nodes={scale=0.55, transform shape}, font=\tiny, legend cell align=left},
    every axis/.append style={line width=0.5pt}
}

%legend pos=outer north east
%legend pos=north west
%legend pos=north east

      \begin{tikzpicture}
              \begin{semilogyaxis}[xlabel=SNR (dB),
            ,ylabel=BLER,
            %legend pos=south west,
            legend columns=2,
            legend style={at={(0.5,1.02)},anchor=south},
            grid=both, xmin=-10,xmax=5, ymin=0.001,ymax=0.3]



\addplot+[smooth,teal, dotted, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
(-3,	0.1345)
(-2,	0.0624)
(-1,	0.0248)
(0	,0.0075)
(1	,0.0012)
(2	,0.0003)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=2}

\addplot+[smooth,teal, dashed, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
%(-6,	0.2021)
(-5,	0.0969)
(-4,	0.036)
(-3,	0.0122)
(-2,	0.0025)
(-1,	0.0002)
(0	,0.0001)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=4}


\addplot+[smooth,teal, solid, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
%(-8,	0.185)
(-7,	0.0799)
(-6,	0.0246)
(-5,	0.0053)
(-4,	0.0009)
(-3,	0.0001)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=8}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%deja bon%%%%%%%%%%
\addplot+[smooth, dotted, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
(-2,	0.1681)
(-1,	0.0999)
(0	,0.0493)
(1	,0.019)
(2	,0.0063)
(3	,0.0014)
(4	,0.0003)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=2}

\addplot+[smooth, dashed, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
(-4,	0.1297)
(-3,	0.0645)
(-2,	0.029)
(-1,	0.0087)
(0	,0.0016)
(1	,0.0004)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=4}

\addplot+[smooth, solid, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
(-6,	0.1129)
(-5,	0.0481)
(-4,	0.012)
(-3,	0.0027)
(-2,	0.0008)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=8}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot+[smooth, dotted, olive, mark options={ scale=1, fill=olive, solid},mark=otimes] coordinates {
(-2,	0.1681)
(-1,	0.0999)
(0	,0.0493)
(1	,0.019)
(2	,0.0063)
(3	,0.0014)
(4	,0.0003)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2}


\addplot+[smooth, dashed, olive, mark options={ scale=1, fill=olive, solid },mark=otimes] coordinates {
(-4,	0.1297)
(-3,	0.0645)
(-2,	0.029)
(-1,	0.0087)
(0	,0.0016)
(1	,0.0004)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4}

\addplot+[smooth, solid, olive, mark options={ scale=1, fill=olive},mark=otimes] coordinates {
(-6,	0.1129)
(-5,	0.0481)
(-4,	0.012)
(-3,	0.0027)
(-2,	0.0008)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot+[smooth,orange, dotted, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-2,	0.1425)
(-1,	0.0824)
(0	,0.0382)
(1	,0.0146)
(2	,0.0052)
(3	,0.0011)
(4	,0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2, $\beta = 1.25$}

\addplot+[smooth,orange, dashed, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-5,	0.1834)
(-4,	0.0995)
(-3,	0.0446)
(-2,	0.0182)
(-1,	0.0045)
(0	,0.0011)
(1	,0.0003)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4, $\beta = 1.25$}

\addplot+[smooth,orange, solid, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-7,	0.148)
(-6,	0.0754)
(-5,	0.0269)
(-4,	0.0063)
(-3,	0.0008)
(-2,	0.0006)

};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8, $\beta = 1.25$}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot+[smooth,green, dotted, mark options={scale=1, fill=green, solid},mark=]coordinates {
(-2,	0.1276)
(-1,	0.0727)
(0	,0.033)
(1	,0.0125)
(2	,0.0046)
(3	,0.0009)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2, $\beta = 1.50$}


\addplot+[smooth,green, dashed, mark options={scale=1, fill=green, solid},mark=]coordinates {
%(-6, 	0.1851)
(-5,	0.1575)
(-4,	0.0824)
(-3,	0.0352)
(-2,	0.0149)
(-1,	0.0038)
(0	,0.0008)
(1	,0.0002)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4, $\beta = 1.50$}

\addplot+[smooth,green, solid, mark options={scale=1, fill=green, solid},mark=]coordinates {
(-7,	0.1149)
(-6,	0.0572)
(-5,	0.019)
(-4,	0.0039)
(-3,	0.0006)
(-2,	0.0002)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8, $\beta = 1.50$}
%
%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\addplot+[smooth,cyan, dotted, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
(-2,	0.1207)
(-1,	0.0677)
(0	,0.0307)
(1	,0.0114)
(2	,0.0042)
(3	,0.001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=2, $\beta = 1.75$}
%
\addplot+[smooth,cyan, dashed, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
%-7	0.2666)
(-5,	0.1414)
(-4,	0.073)
(-3,	0.0314)
(-2,	0.0123)
(-1,	0.003)
(0	,0.0004)
(1	,0.0001)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4, $\beta = 1.75$}
%
%
\addplot+[smooth,cyan, solid, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
%(-8,	0.1835)
(-7,	0.0976)
(-6,	0.0467)
(-5,	0.0155)
(-4,	0.0034)
(-3,	0.0004)
(-2,	0.0002)

};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=8, $\beta = 1.75$}

%%%%%%%
        \end{semilogyaxis}
    \end{tikzpicture}


==> figures/tikz/ray/new_tdl_scalled.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.74902,0.74902,0.00000}%
\definecolor{mycolor2}{rgb}{0.74902,0.00000,0.74902}%
\definecolor{mycolor3}{rgb}{0.85098,0.32549,0.09804}%
\definecolor{mycolor4}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor5}{rgb}{0.46667,0.67451,0.18824}%
%
\begin{tikzpicture}

\begin{axis}[%
width=10.301in,
height=7.267in,
at={(1.728in,0.981in)},
scale only axis,
xmin=-10,
xmax=5,
ymode=log,
ymin=0.001,
ymax=0.5,
yminorticks=true,
axis background/.style={fill=white},
xminorgrids,
yminorgrids,
minor grid style={solid},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=1.0pt, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9875\\
-13	0.9803\\
-12	0.9681\\
-11	0.9466\\
-10	0.9087\\
-9	0.8638\\
-8	0.7822\\
-7	0.671\\
-6	0.5352\\
-5	0.3781\\
-4	0.2344\\
-3	0.1345\\
-2	0.0624\\
-1	0.0248\\
0	0.0075\\
1	0.0012\\
2	0.0003\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, 3GPP RM Codes, Quasi Coherent ML DEC., nRx=2}

\addplot [color=mycolor1, line width=1.0pt, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9706\\
-13	0.9522\\
-12	0.9203\\
-11	0.8669\\
-10	0.793\\
-9	0.6708\\
-8	0.5198\\
-7	0.3528\\
-6	0.2021\\
-5	0.0969\\
-4	0.036\\
-3	0.0122\\
-2	0.0025\\
-1	0.0002\\
0	0.0001\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, 3GPP RM Codes, Quasi Coherent ML DEC., nRx=4}

\addplot [color=mycolor1, line width=1.0pt, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9367\\
-13	0.8808\\
-12	0.8023\\
-11	0.6854\\
-10	0.5191\\
-9	0.3488\\
-8	0.185\\
-7	0.0799\\
-6	0.0246\\
-5	0.0053\\
-4	0.0009\\
-3	0.0001\\
-2	0\\
-1	0\\
0	0\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, 3GPP RM Codes, Quasi Coherent ML DEC., nRx=8}

\addplot [color=mycolor2, line width=1.0pt, mark=square, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9222\\
-13	0.9084\\
-12	0.8895\\
-11	0.8637\\
-10	0.8332\\
-9	0.7873\\
-8	0.729\\
-7	0.6734\\
-6	0.5784\\
-5	0.4821\\
-4	0.3688\\
-3	0.2789\\
-2	0.1681\\
-1	0.0999\\
0	0.0493\\
1	0.019\\
2	0.0063\\
3	0.0014\\
4	0.0003\\
5	0\\
};
\addlegendentry{11 bits, Block-based RM Coding, Dec. via FHT, nRx=2}

\addplot [color=mycolor2, line width=1.0pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8941\\
-13	0.8759\\
-12	0.8346\\
-11	0.7951\\
-10	0.7414\\
-9	0.6715\\
-8	0.5709\\
-7	0.4662\\
-6	0.3425\\
-5	0.2281\\
-4	0.1297\\
-3	0.0645\\
-2	0.029\\
-1	0.0087\\
0	0.0016\\
1	0.0004\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, Block-based RM Coding, Dec. via FHT, nRx=4}

\addplot [color=mycolor2, line width=1.0pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8516\\
-13	0.8081\\
-12	0.7462\\
-11	0.6738\\
-10	0.5727\\
-9	0.457\\
-8	0.3334\\
-7	0.2069\\
-6	0.1129\\
-5	0.0481\\
-4	0.012\\
-3	0.0027\\
-2	0.0008\\
-1	0\\
0	0\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, Block-based RM Coding, Dec. via FHT, nRx=8}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8992\\
-13	0.8765\\
-12	0.8485\\
-11	0.8157\\
-10	0.7781\\
-9	0.7178\\
-8	0.6537\\
-7	0.5835\\
-6	0.4971\\
-5	0.3984\\
-4	0.2911\\
-3	0.2092\\
-2	0.1207\\
-1	0.0677\\
0	0.0307\\
1	0.0114\\
2	0.0042\\
3	0.001\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=2, }\beta\text{=1.75}$}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
-15	0\\
-14	0.7695\\
-13	0.7024\\
-12	0.6111\\
-11	0.5202\\
-10	0.4015\\
-9	0.2891\\
-8	0.1835\\
-7	0.0976\\
-6	0.0467\\
-5	0.0155\\
-4	0.0034\\
-3	0.0004\\
-2	0.0002\\
-1	0\\
0	0\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=8, }\beta\text{=1.75}$}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8512\\
-13	0.8211\\
-12	0.7625\\
-11	0.7011\\
-10	0.6484\\
-9	0.5467\\
-8	0.4401\\
-7	0.3325\\
-6	0.2256\\
-5	0.1414\\
-4	0.073\\
-3	0.0314\\
-2	0.0123\\
-1	0.003\\
0	0.0004\\
1	0.0001\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=4, }\beta\text{=1.75}$}

\addplot [color=mycolor4, line width=1.0pt, mark=asterisk, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
-15	0\\
-14	0.7934\\
-13	0.7318\\
-12	0.6485\\
-11	0.5634\\
-10	0.4395\\
-9	0.3246\\
-8	0.2128\\
-7	0.1149\\
-6	0.0572\\
-5	0.019\\
-4	0.0039\\
-3	0.0006\\
-2	0.0002\\
-1	0\\
0	0\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=8, }\beta\text{=1.50}$}

\addplot [color=mycolor4, line width=1.0pt, mark=asterisk, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9068\\
-13	0.887\\
-12	0.8612\\
-11	0.8285\\
-10	0.7939\\
-9	0.7359\\
-8	0.6689\\
-7	0.5998\\
-6	0.5133\\
-5	0.4144\\
-4	0.3054\\
-3	0.2218\\
-2	0.1276\\
-1	0.0727\\
0	0.033\\
1	0.0125\\
2	0.0046\\
3	0.0009\\
4	0\\
5	0.0001\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=2, }\beta\text{=1.50}$}

\addplot [color=mycolor4, line width=1.0pt, mark=asterisk, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8671\\
-13	0.8372\\
-12	0.7831\\
-11	0.7259\\
-10	0.6734\\
-9	0.5763\\
-8	0.4716\\
-7	0.3633\\
-6	0.2454\\
-5	0.1575\\
-4	0.0824\\
-3	0.0352\\
-2	0.0149\\
-1	0.0038\\
0	0.0008\\
1	0.0002\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=4, }\beta\text{=1.50}$}

\addplot [color=mycolor5, line width=1.0pt, mark=asterisk, mark options={solid, mycolor5}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8228\\
-13	0.769\\
-12	0.6908\\
-11	0.613\\
-10	0.4985\\
-9	0.3759\\
-8	0.2588\\
-7	0.148\\
-6	0.0754\\
-5	0.0269\\
-4	0.0063\\
-3	0.0008\\
-2	0.0006\\
-1	0\\
0	0\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=8, }\beta\text{=1.25}$}

\addplot [color=mycolor5, line width=1.0pt, mark=asterisk, mark options={solid, mycolor5}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9138\\
-13	0.8954\\
-12	0.8759\\
-11	0.8433\\
-10	0.8132\\
-9	0.7586\\
-8	0.6956\\
-7	0.6312\\
-6	0.5395\\
-5	0.4421\\
-4	0.3305\\
-3	0.2424\\
-2	0.1425\\
-1	0.0824\\
0	0.0382\\
1	0.0146\\
2	0.0052\\
3	0.0011\\
4	0.0001\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=2, }\beta\text{=1.25}$}

\addplot [color=mycolor5, line width=1.0pt, mark=asterisk, mark options={solid, mycolor5}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8794\\
-13	0.8545\\
-12	0.8076\\
-11	0.7584\\
-10	0.704\\
-9	0.6155\\
-8	0.5112\\
-7	0.4058\\
-6	0.2829\\
-5	0.1834\\
-4	0.0995\\
-3	0.0446\\
-2	0.0182\\
-1	0.0045\\
0	0.0011\\
1	0.0003\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, Block-based RM Coding, Dec. via FHT, nRx=4, }\beta\text{=1.25}$}

\end{axis}
\end{tikzpicture}%

==> figures/tikz/save/comp_new_rx.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.87059,0.49020,0.00000}%
\definecolor{mycolor2}{rgb}{0.74902,0.74902,0.00000}%
\definecolor{mycolor3}{rgb}{0.60000,0.20000,0.00000}%
\definecolor{mycolor4}{rgb}{0.30196,0.74510,0.93333}%
\begin{tikzpicture}[scale=.6, transform shape]

\begin{axis}[%
  width=4.8in,
  height=4in,
at={(2.158in,2.261in)},
scale only axis,
xmin=-10,
xmax=2,
xlabel style={font=\color{white!15!black}},
xlabel={SNR ( dB )},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={BLER},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
minor grid style={solid},
legend style={at={(0.326,0.820)}, anchor=south west, legend cell align=left, align=left, font=\small, draw=white!15!black}
]
% \addplot [color=mycolor1, mark=*, mark options={solid, fill=mycolor1, draw=mycolor1}]
%   table[row sep=crcr]{%
% -15	0\\
% -14	0.7078\\
% -13	0.635\\
% -12	0.5561\\
% -11	0.4511\\
% -10	0.3455\\
% -9	0.2498\\
% -8	0.1605\\
% -7	0.0945\\
% -6	0.0502\\
% -5	0.0233\\
% -4	0.0083\\
% -3	0.0022\\
% -2	0.0003\\
% -1	0.0002\\
% 0	0\\
% 1	0\\
% 2	0\\
% 3	0\\
% 4	0\\
% 5	0\\
% };
% \addlegendentry{11 bits, 3GPP Standard RM codes,   ML Dec., nRx=4}

\addplot [color=mycolor2, mark=*, mark options={solid, fill=mycolor2, draw=mycolor2}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9705\\
-13	0.9509\\
-12	0.9146\\
-11	0.8551\\
-10	0.7733\\
-9	0.6495\\
-8	0.4939\\
-7	0.3392\\
-6	0.2016\\
-5	0.1073\\
-4	0.0422\\
-3	0.0172\\
-2	0.0043\\
-1	0.001\\
0	0.0002\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, 3GPP Standard RM codes,   ML Dec., nRx=4}
%\addlegendentry{11 bits, Block-based Coding, ML DEC., nRx=4}

\addplot [color=mycolor3, mark=*, mark options={solid, fill=mycolor3, draw=mycolor3}]
  table[row sep=crcr]{%
-15	0\\
-14	0.907\\
-13	0.8762\\
-12	0.8391\\
-11	0.7875\\
-10	0.7378\\
-9	0.6589\\
-8	0.5502\\
-7	0.4381\\
-6	0.3096\\
-5	0.196\\
-4	0.1043\\
-3	0.0464\\
-2	0.0182\\
-1	0.0041\\
0	0.0011\\
1	0.0001\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, RM Codes, Block-based  Dec. via HT, nRx=4}

\addplot [color=mycolor4, mark=*, mark options={solid, fill=mycolor4, draw=mycolor4}]
  table[row sep=crcr]{%
-15	0\\
-14	0.907\\
-13	0.8762\\
-12	0.8391\\
-11	0.7875\\
-10	0.7378\\
-9	0.6589\\
-8	0.5502\\
-7	0.4381\\
-6	0.3096\\
-5	0.196\\
-4	0.1043\\
-3	0.0464\\
-2	0.0182\\
-1	0.0041\\
0	0.0011\\
1	0.0001\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, RM Codes, Block-based  Dec. via FHT, nRx=4}

\end{axis}
\end{tikzpicture}%


==> figures/tikz/save/comp_optim.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.87059,0.49020,0.00000}%
\definecolor{mycolor2}{rgb}{0.74902,0.74902,0.00000}%
\definecolor{mycolor3}{rgb}{0.60000,0.20000,0.00000}%
\definecolor{mycolor4}{rgb}{0.30196,0.74510,0.93333}%
\definecolor{mycolor5}{rgb}{0.90000.80000,0.18824}%
\definecolor{mycolor6}{rgb}{0.49412,0.18431,0.55686}%
\begin{tikzpicture}[scale=.6, transform shape]

\begin{axis}[%
  width=4.8in,
  height=4in,
at={(2.158in,2.261in)},
scale only axis,
xmin=-10,
xmax=2,
xlabel style={font=\color{white!15!black}},
xlabel={SNR ( dB )},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={BLER},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
minor grid style={solid},
legend style={at={(0.230,0.746)}, anchor=south west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black}
]
%\footnotesize
%scriptsize
% \addplot [color=mycolor1, mark=*, mark options={solid, fill=mycolor1, draw=mycolor1}]
%   table[row sep=crcr]{%
% -15	0\\
% -14	0.7078\\
% -13	0.635\\
% -12	0.5561\\
% -11	0.4511\\
% -10	0.3455\\
% -9	0.2498\\
% -8	0.1605\\
% -7	0.0945\\
% -6	0.0502\\
% -5	0.0233\\
% -4	0.0083\\
% -3	0.0022\\
% -2	0.0003\\
% -1	0.0002\\
% 0	0\\
% 1	0\\
% 2	0\\
% 3	0\\
% 4	0\\
% 5	0\\
% };
% \addlegendentry{11 bits, 3GPP RM codes,   ML Dec., nRx=4}

\addplot [color=mycolor2, mark=*, mark options={solid, fill=mycolor2, draw=mycolor2}]
  table[row sep=crcr]{%
-15	0\\
-14	0.9705\\
-13	0.9509\\
-12	0.9146\\
-11	0.8551\\
-10	0.7733\\
-9	0.6495\\
-8	0.4939\\
-7	0.3392\\
-6	0.2016\\
-5	0.1073\\
-4	0.0422\\
-3	0.0172\\
-2	0.0043\\
-1	0.001\\
0	0.0002\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
%\addlegendentry{11 bits, RM codes, Block-based Coding, ML DEC., nRx=4}
\addlegendentry{11 bits, 3GPP RM codes,   ML Dec., nRx=4}

\addplot [color=mycolor3, mark=*, mark options={solid, fill=mycolor3, draw=mycolor3}]
  table[row sep=crcr]{%
-15	0\\
-14	0.907\\
-13	0.8762\\
-12	0.8391\\
-11	0.7875\\
-10	0.7378\\
-9	0.6589\\
-8	0.5502\\
-7	0.4381\\
-6	0.3096\\
-5	0.196\\
-4	0.1043\\
-3	0.0464\\
-2	0.0182\\
-1	0.0041\\
0	0.0011\\
1	0.0001\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, RM codes, Block-based Coding, Dec. via HT, nRx=4}

\addplot [color=mycolor4, mark=*, mark options={solid, fill=mycolor4, draw=mycolor4}]
  table[row sep=crcr]{%
-15	0\\
-14	0.907\\
-13	0.8762\\
-12	0.8391\\
-11	0.7875\\
-10	0.7378\\
-9	0.6589\\
-8	0.5502\\
-7	0.4381\\
-6	0.3096\\
-5	0.196\\
-4	0.1043\\
-3	0.0464\\
-2	0.0182\\
-1	0.0041\\
0	0.0011\\
1	0.0001\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{11 bits, RM codes, Block-based Coding Dec. via FHT, nRx=4}

\addplot [color=black, dashdotted, mark=+, mark options={solid, fill=black, draw=black}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8849\\
-13	0.8491\\
-12	0.8036\\
-11	0.7419\\
-10	0.6809\\
-9	0.5854\\
-8	0.4704\\
-7	0.3488\\
-6	0.2314\\
-5	0.1346\\
-4	0.0632\\
-3	0.0265\\
-2	0.009\\
-1	0.0021\\
0	0.0005\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, RM codes, Block-based Dec. via FHT, nRx=4, }\beta\text{=1.25}$}

\addplot [color=mycolor5, dotted, mark=star*, mark options={solid, fill=mycolor5, draw=mycolor5}]
  table[row sep=crcr]{%
-15	0\\
-14	0.8628\\
-13	0.825\\
-12	0.7758\\
-11	0.7011\\
-10	0.6367\\
-9	0.5235\\
-8	0.4115\\
-7	0.294\\
-6	0.186\\
-5	0.1046\\
-4	0.048\\
-3	0.0197\\
-2	0.0058\\
-1	0.0014\\
0	0.0002\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, RM codes, Block-based  Dec. via FHT, nRx=4, }\beta\text{=1.5}$}

\addplot [color=mycolor6, dashed, mark=asterisk, mark options={solid, fill=mycolor6, draw=mycolor6}]
  table[row sep=crcr]{%
-15	0\\
-14	0.848\\
-13	0.8044\\
-12	0.7493\\
-11	0.6676\\
-10	0.5987\\
-9	0.482\\
-8	0.3728\\
-7	0.2666\\
-6	0.16\\
-5	0.0912\\
-4	0.0409\\
-3	0.0152\\
-2	0.0051\\
-1	0.0013\\
0	0.0002\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
};
\addlegendentry{$\text{11 bits, RM codes, Block-based Coding, Dec. via FHT, nRx=4, }\beta\text{=1.75}$}

\end{axis}

\end{tikzpicture}%


==> figures/tikz/save/fht_decoder_mL.tex <==
% % Preamble:
%  \pgfplotsset{width=7cm,compat=newest} \pgfplotsset{every axis/.append style={
%     font=\footnotesize,
%     thin,
%     tick style={ultra thin}}}
% \begin{tikzpicture}[scale=0.5]
%     \begin{loglogaxis}[
%         xlabel=\textsc{Dof},
%         ylabel=$L_2$ Error
%     ]
%     %  see above for this macro:
%     \plotcoords
%     \legend{$d=2$,$d=3$,$d=4$,$d=5$,$d=6$}
%     \end{loglogaxis}
% \end{tikzpicture}

% \begin{tikzpicture}
%         \begin{semilogyaxis}[xlabel=SNR (dB),
%       ,ylabel=BLER, xmin=0,xmax=20, ymin=1e-5,ymax=1]
\pgfplotsset{
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    legend style={nodes={scale=0.7, transform shape}, font=\tiny, legend cell align=left},
    every axis/.append style={line width=0.5pt}
}



%legend pos=outer north east
%legend pos=north west
%legend pos=north east

\begin{tikzpicture}
              \begin{semilogyaxis}[xlabel=SNR (dB),
            ,ylabel=BLER, xmin=-7,xmax=1, ymin=1e-3,ymax=0.5, legend pos=north east,
            grid=both,
            ]

\addplot+[smooth,teal, dashed, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
(-6,	0.2016)
(-5,	0.1073)
(-4,	0.0422)
(-3,	0.0172)
(-2,	0.0043)
(-1,	0.001)
(0,	0.0002)
(1,	0)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=4}

\addplot+[smooth, dashdotted, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
(-5,	0.196)
(-4,	0.1043)
(-3,	0.0464)
(-2,	0.0182)
(-1,	0.0041)
(0,	0.0011)
(1,	0.0001)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=4}

\addplot+[smooth, solid, olive, mark options={ scale=1, fill=olive},mark=otimes] coordinates {
(-5,	0.196)
(-4,	0.1043)
(-3,	0.0464)
(-2,	0.0182)
(-1,	0.0041)
(0,	0.0011)
(1,	0.0001)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \addplot+[smooth,orange, dashed, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
% (-6,	0.2314)
% (-5,	0.1346)
% (-4,	0.0632)
% (-3,	0.0265)
% (-2,	0.009)
% (-1,	0.0021)
% (0,	0.0005)
% (1,	0)
% (2,	0)
% (3,	0)
% (4,	0)
% (5,	0)
% };
% \addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, $\beta = 1.25$}
%
%
%
% \addplot+[smooth,green, dashed, mark options={scale=1, fill=green, solid},mark=]coordinates {
% (-6,	0.186)
% (-5,	0.1046)
% (-4,	0.048)
% (-3,	0.0197)
% (-2,	0.0058)
% (-1,	0.0014)
% (0,	0.0002)
% (1,	0)
% (2,	0)
% (3,	0)
% (4,	0)
% (5,	0)
% };
% \addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, $\beta = 1.50$}
%
% \addplot+[smooth,cyan, dashed, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
% %-7	0.2666)
% (-6,	0.16)
% (-5,	0.0912)
% (-4,	0.0409)
% (-3,	0.0152)
% (-2,	0.0051)
% (-1,	0.0013)
% (0,	0.0002)
% (1,	0)
% (2,	0)
% (3,	0)
% (4,	0)
% (5,	0)
% };
% \addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, $\beta = 1.75$}

%%%%%%%
        \end{semilogyaxis}
    \end{tikzpicture}


==> figures/tikz/save/fht_decoder_optim.tex <==
% % Preamble:
%  \pgfplotsset{width=7cm,compat=newest} \pgfplotsset{every axis/.append style={
%     font=\footnotesize,
%     thin,
%     tick style={ultra thin}}}
% \begin{tikzpicture}[scale=0.5]
%     \begin{loglogaxis}[
%         xlabel=\textsc{Dof},
%         ylabel=$L_2$ Error
%     ]
%     %  see above for this macro:
%     \plotcoords
%     \legend{$d=2$,$d=3$,$d=4$,$d=5$,$d=6$}
%     \end{loglogaxis}
% \end{tikzpicture}

% \begin{tikzpicture}
%         \begin{semilogyaxis}[xlabel=SNR (dB),
%       ,ylabel=BLER, xmin=0,xmax=20, ymin=1e-5,ymax=1]
\pgfplotsset{
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    legend style={nodes={scale=0.7, transform shape}, font=\tiny, legend cell align=left},
    every axis/.append style={line width=0.5pt}
}



%legend pos=outer north east
%legend pos=north west
%legend pos=north east

\begin{tikzpicture}
              \begin{semilogyaxis}[xlabel=SNR (dB),
            ,ylabel=BLER, xmin=-7,xmax=1, ymin=1e-3,ymax=0.5, legend pos=north east,
            grid=both,
            ]

\addplot+[smooth,teal, dashed, mark options={scale=1, fill=teal, solid},mark=oplus] coordinates {
(-6,	0.2016)
(-5,	0.1073)
(-4,	0.0422)
(-3,	0.0172)
(-2,	0.0043)
(-1,	0.001)
(0,	0.0002)
(1,	0)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, 3GPP RM$\sim \mathcal C(32,11)$,  ML Dec., nRx=4}

\addplot+[smooth, dashdotted, red, mark options={ scale=1, fill=red, solid},mark=square] coordinates {
(-5,	0.196)
(-4,	0.1043)
(-3,	0.0464)
(-2,	0.0182)
(-1,	0.0041)
(0,	0.0011)
(1,	0.0001)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM , Dec. via HT, nRx=4}

\addplot+[smooth, solid, olive, mark options={ scale=1, fill=olive},mark=otimes] coordinates {
(-5,	0.196)
(-4,	0.1043)
(-3,	0.0464)
(-2,	0.0182)
(-1,	0.0041)
(0,	0.0011)
(1,	0.0001)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, nRx=4}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot+[smooth,orange, dashed, mark options={scale=1, fill=orange, solid},mark=asterisk] coordinates {
(-6,	0.2314)
(-5,	0.1346)
(-4,	0.0632)
(-3,	0.0265)
(-2,	0.009)
(-1,	0.0021)
(0,	0.0005)
(1,	0)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, $\beta = 1.25$}



\addplot+[smooth,green, dashed, mark options={scale=1, fill=green, solid},mark=]coordinates {
(-6,	0.186)
(-5,	0.1046)
(-4,	0.048)
(-3,	0.0197)
(-2,	0.0058)
(-1,	0.0014)
(0,	0.0002)
(1,	0)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, $\beta = 1.50$}

\addplot+[smooth,cyan, dashed, mark options={scale=1, fill=cyan, solid},mark=|]coordinates {
%-7	0.2666)
(-6,	0.16)
(-5,	0.0912)
(-4,	0.0409)
(-3,	0.0152)
(-2,	0.0051)
(-1,	0.0013)
(0,	0.0002)
(1,	0)
(2,	0)
(3,	0)
(4,	0)
(5,	0)
};
\addlegendentry{11 bits, Block-based RM Enc. , Dec. via FHT, $\beta = 1.75$}

%%%%%%%
        \end{semilogyaxis}
    \end{tikzpicture}


==> figures/tikzfigure/propose0.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.49412,0.18431,0.55686}%
\definecolor{mycolor2}{rgb}{0.14902,0.14902,0.14902}%
%

\begin{tikzpicture}[scale=.55, transform shape]
\begin{axis}[%
width=5.5in,
height=4.4in,
at={(1.887in,0.898in)},
%at={(1.02in,2.274in)},
scale only axis,
xmin=-12,
xmax=2,
xlabel style={font=\color{white!18!black}},
xlabel={SNR per RE (dB)},
ymode=log,
ymin=0.009,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!18!black}},
ylabel={$\text{P}_\text{e}$},
axis background/.style={fill=white},
xminorgrids,
yminorgrids,
minor grid style={solid},
%legend style={at={(0.38,0.01)}, anchor=south west, legend cell align=left, align=left, draw=blue!15!black}
legend style={legend cell align=left, align=left, draw=white!10!black}
]
\addplot [color=mycolor1, mark=square*, mark options={solid, fill=mycolor1, draw=mycolor1}]
  table[row sep=crcr]{%
-10	0.8162\\
-9	0.6967\\
-8	0.5447\\
-7	0.3701\\
-6	0.1955\\
-5	0.0868\\
-4	0.0254\\
-3	0.00514509158263017\\
-2	0.00091\\
-1	0.00019\\
};
\addlegendentry{non-coherent ML receiver, 4 Rx antennas}

\addplot [color=black, dotted, line width=1.0pt, mark=square*, mark options={solid, fill=black, draw=black}]
  table[row sep=crcr]{%
-10	0.8983\\
-9	0.8209\\
-8	0.6952\\
-7	0.535\\
-6	0.3613\\
-5	0.1911\\
-4	0.0791\\
-3	0.0222\\
-2	0.00376010528294792\\
-1	0.00057\\
};
\addlegendentry{conventional receiver, 4 Rx antennas}

\addplot [color=mycolor1, mark=asterisk, mark options={solid, fill=mycolor1, draw=mycolor1}]
  table[row sep=crcr]{%
-15	0.9937\\
-14	0.9895\\
-13	0.9859\\
-12	0.9794\\
-11	0.9621\\
-10	0.9411\\
-9	0.8996\\
-8	0.8425\\
-7	0.7455\\
-6	0.6308\\
-5	0.4557\\
-4	0.2986\\
-3	0.1672\\
-2	0.0691\\
-1	0.0242\\
0	0.00847816871555744\\
1	0.00297159158445263\\
2	0.00108536386823683\\
3	0.00048\\
4	0.00012\\
5	0.0001\\
6	3e-05\\
};
\addlegendentry{non-coherent ML receiver, 2 Rx antennas}

\addplot [color=black, dotted, line width=1.0pt, mark=asterisk, mark options={solid, fill=black, draw=black}]
  table[row sep=crcr]{%
-10	0.9541\\
-9	0.9316\\
-8	0.8848\\
-7	0.8174\\
-6	0.7093\\
-5	0.5651\\
-4	0.4043\\
-3	0.246\\
-2	0.1168\\
-1	0.0483\\
0	0.0159\\
1	0.00359259924555416\\
2	0.00088\\
};
\addlegendentry{conventional receiver, 2 Rx antennas}

\addplot [color=mycolor1, mark=*, mark options={solid, fill=mycolor1, draw=mycolor1}]
  table[row sep=crcr]{%
-12	0.8189\\
-11	0.6806\\
-10	0.498\\
-9	0.2911\\
-8	0.1331\\
-7	0.0431\\
-6	0.00817795224075891\\
-5	0.00106971320988843\\
-4	4e-05\\
-3	1e-05\\
};
\addlegendentry{non-coherent ML receiver, 8 Rx antennas}

\addplot [color=black, dotted, line width=1.0pt, mark=*, mark options={solid, fill=black, draw=black}]
  table[row sep=crcr]{%
-12	0.9028\\
-11	0.8323\\
-10	0.6977\\
-9	0.5398\\
-8	0.3337\\
-7	0.1683\\
-6	0.0571\\
-5	0.0132\\
-4	0.00133854473416502\\
-3	7e-05\\
};
\addlegendentry{conventional receiver, 8 Rx antennas}

% \end{axis}
%
% \begin{axis}[%
% width=7.847in,
% height=9.903in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
\end{axis}
\end{tikzpicture}%


==> figures/tikzfigure/propose1.tex <==

\definecolor{mycolor1}{rgb}{0.49412,0.18431,0.55686}%
\definecolor{mycolor2}{rgb}{0.74902,0.74902,0.00000}%
\definecolor{mycolor3}{rgb}{0.00000,0.44706,0.74118}%
\definecolor{mycolor4}{rgb}{0.16471,0.38431,0.27451}%
\definecolor{mycolor5}{rgb}{0.10588,0.30980,0.20784}%
\definecolor{mycolor6}{rgb}{0.14902,0.14902,0.14902}%
%
\begin{tikzpicture}[scale=.6, transform shape]
\begin{axis}[%
width=5in,
height=4in,
at={(1.887in,0.898in)},
scale only axis,
xmin=-10,
xmax=0,
xlabel style={font=\color{white!18!black}},
xlabel={SNR per RE (dB)},
ymode=log,
ymin=10^-3.5,
ymax=10^0,
yminorticks=true,
ylabel style={font=\color{white!18!black}},
ylabel={$\text{P}_\text{e}$},
axis background/.style={fill=white},
xminorgrids,
yminorgrids,
minor grid style={solid},
%legend style={at={(0.38,0.01)}, anchor=south west, legend cell align=left, align=left, draw=blue!15!black}
legend style={legend cell align=left, align=left, draw=white!10!black}
]
\addplot [color=mycolor1, mark=square*, mark options={solid, fill=mycolor1, draw=mycolor1}]
  table[row sep=crcr]{%
-10	0.8162\\
-9	0.6967\\
-8	0.5447\\
-7	0.3701\\
-6	0.1955\\
-5	0.0868\\
-4	0.0254\\
-3	0.00514509158263017\\
-2	0.00091\\
-1	0.00019\\
};
\addlegendentry{reference non-coherent receiver, 4 Rx antennas}

\addplot [color=black, dotted, line width=1.0pt, mark=square*, mark options={solid, fill=black, draw=black}]
  table[row sep=crcr]{%
-10	0.8983\\
-9	0.8209\\
-8	0.6952\\
-7	0.535\\
-6	0.3613\\
-5	0.1911\\
-4	0.0791\\
-3	0.0222\\
-2	0.00376010528294792\\
-1	0.00057\\
};
\addlegendentry{conventional receiver, 4 Rx antennas}

\addplot [color=mycolor2, dashdotted, mark=asterisk, mark options={solid, fill=mycolor2, draw=mycolor2}]
  table[row sep=crcr]{%
-10	0.8018\\
-9	0.6725\\
-8	0.5135\\
-7	0.3187\\
-6	0.1749\\
-5	0.0593\\
-4	0.0159\\
-3	0.00365550519081737\\
-2	0.00053\\
-1	6e-05\\
0	3e-05\\
1	0\\
2	0\\
};
\addlegendentry{enhanced receiver, 4 Rx antennas (.75 DMRS power)}

\addplot [color=mycolor3, dashdotted, mark=triangle*, mark options={solid, fill=mycolor3, draw=mycolor3}]
  table[row sep=crcr]{%
-10	0.7721\\
-9	0.6467\\
-8	0.4746\\
-7	0.2877\\
-6	0.1365\\
-5	0.0453\\
-4	0.0132\\
-3	0.00183392018779343\\
-2	0.00029\\
-1	6e-05\\
0	0\\
1	0\\
2	0\\
};
\addlegendentry{enhanced receiver, 4 Rx antennas (.5 DMRS power)}

\addplot [color=mycolor4, dashdotted, mark=*, mark options={solid, fill=mycolor4, draw=mycolor5}]
  table[row sep=crcr]{%
-10	0.7654\\
-9	0.6291\\
-8	0.4485\\
-7	0.2657\\
-6	0.1272\\
-5	0.0476\\
-4	0.0134\\
-3	0.00267766293578964\\
-2	0.00077\\
-1	0.00017\\
0	2e-05\\
1	0\\
2	0\\
};
\addlegendentry{enhanced receiver, 4 Rx antennas, (.25 DMRS power)}

\end{axis}
\end{tikzpicture}%


==> figures/tikzfigure/pucch2_3gpp_.tex <==


\tikzset{every picture/.style={line width=0.25pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,423); %set diagram left start at 0, and has height of 423

%Shape: Rectangle [id:dp534691631513805]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (146,297) -- (163,297) -- (163,372.8) -- (146,372.8) -- cycle ;
%Shape: Rectangle [id:dp6022279546278549]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (190.83,328.15) -- (251.83,328.15) -- (251.83,339.67) -- (190.83,339.67) -- cycle ;
%Shape: Rectangle [id:dp5166149169364767]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (308,328.15) -- (354.83,328.15) -- (354.83,339.67) -- (308,339.67) -- cycle ;
%Shape: Rectangle [id:dp42623882906925825]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (377,327.67) -- (452.19,327.67) -- (452.19,339.65) -- (377,339.65) -- cycle ;
%Straight Lines [id:da8477777336257208]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (70,320) -- (141.25,320.17) ;
\draw [shift={(144.25,320.17)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da18217775366174027]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (68,351) -- (142.25,351.17) ;
\draw [shift={(145.25,351.17)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da91367637045185]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (163,334) -- (188.25,334.16) ;
\draw [shift={(191.25,334.17)}, rotate = 180.35] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da6524188236465472]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (252,334) -- (268.5,334) ;
\draw [shift={(271.5,334)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da4038350534737931]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (283.5,334) -- (306.17,334.29) ;
\draw [shift={(309.17,334.33)}, rotate = 180.74] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da2642827649455852]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (354.5,334) -- (374.5,334) ;
\draw [shift={(377.5,334)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da4342142667637895]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (452.5,334) -- (469.5,334) ;
\draw [shift={(472.5,334)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da7994657136767602]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (275.8,366.43) -- (275.8,344.43) ;
\draw [shift={(275.8,341.43)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;

% Text Node
\draw (64.77,354) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {System/user params};
% Text Node
\draw (268,328.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\bigotimes $};
% Text Node
\draw (155.99,314.57) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-88.73] [align=center] {RM Encoder};
% Text Node
\draw (198.83,331.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] {Rate Matching};
% Text Node
\draw (315,331.15) node [anchor=north west][inner sep=0.50pt]  [font=\tiny]{Modulation};
% Text Node
\draw (385,330.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]{Ressource Mapping};
% Text Node
\draw (256.77,369) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] {Scrambling};
% Text Node
\draw (71,309.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] {$K$ -message bits};
% Text Node
\draw (456,322.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$x_{m}$};


\end{tikzpicture}


==> figures/tikzfigure/rx_propose.tex <==


\tikzset{every picture/.style={line width=0.25pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,672); %set diagram left start at 0, and has height of 672

%Shape: Rectangle [id:dp22003846932101323]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (24.99,357.15) -- (34.79,357.15) -- (34.79,364.07) -- (24.99,364.07) -- cycle ;
%Shape: Rectangle [id:dp7700006143209311]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (131.99,337) -- (144.11,337) -- (144.11,439.03) -- (131.99,439.03) -- cycle ;
%Shape: Rectangle [id:dp11936228121946613]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (313.82,375.15) -- (358.32,375.15) -- (358.32,397.67) -- (313.82,397.67) -- cycle ;
%Shape: Rectangle [id:dp37631584604893653]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (380.99,377.15) -- (427.82,377.15) -- (427.82,397.67) -- (380.99,397.67) -- cycle ;
%Shape: Rectangle [id:dp40339941132397117]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (449.99,376.67) -- (498.33,376.67) -- (498.33,397.67) -- (449.99,397.67) -- cycle ;
%Straight Lines [id:da3102074746197405]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (31.65,382.65) -- (130.23,382.17) ;
\draw [shift={(28.65,382.67)}, rotate = 359.72] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da15702907324743787]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (288.99,385.02) -- (314.23,385.17) ;
\draw [shift={(285.99,385)}, rotate = 0.35] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da933696111863013]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (430.49,387) -- (450.49,387) ;
\draw [shift={(427.49,387)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da3658932338978075]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (501.49,388) -- (518.49,388) ;
\draw [shift={(498.49,388)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Shape: Rectangle [id:dp8859847686913521]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (173.99,338.15) -- (233.65,338.15) -- (233.65,358) -- (173.99,358) -- cycle ;
%Shape: Rectangle [id:dp6732726240127749]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (34.79,357.15) -- (44.59,357.15) -- (44.59,364.07) -- (34.79,364.07) -- cycle ;
%Shape: Rectangle [id:dp463506101738291]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (44.59,357.15) -- (54.4,357.15) -- (54.4,364.07) -- (44.59,364.07) -- cycle ;
%Shape: Rectangle [id:dp8874180128664084]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (54.4,357.07) -- (63.77,357.07) -- (63.77,364.07) -- (54.4,364.07) -- cycle ;
%Shape: Rectangle [id:dp7653775497361661]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (63.77,357.07) -- (73.14,357.07) -- (73.14,364.07) -- (63.77,364.07) -- cycle ;
%Shape: Rectangle [id:dp7299684567811285]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (73.14,364) -- (80.65,364) -- (80.65,357) -- (73.14,357) -- cycle ;
%Straight Lines [id:da4588392812980727]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (146.65,343.71) -- (173.99,344.15) ;
\draw [shift={(143.65,343.67)}, rotate = 0.91] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da2339171376551623]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (147.65,378.67) -- (175.65,378.67) ;
\draw [shift={(144.65,378.67)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da6387888551032722]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (146.65,426.67) -- (172.65,426.67) ;
\draw [shift={(143.65,426.67)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Shape: Rectangle [id:dp1059816746619685]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (259,339.03) -- (285.11,339.03) -- (285.11,442.03) -- (259,442.03) -- cycle ;
%Shape: Rectangle [id:dp1721021389328855]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (94.4,357.07) -- (103.77,357.07) -- (103.77,364.07) -- (94.4,364.07) -- cycle ;
%Shape: Rectangle [id:dp38225730788537415]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (103.77,357.07) -- (113.14,357.07) -- (113.14,364.07) -- (103.77,364.07) -- cycle ;
%Shape: Rectangle [id:dp44701659314668696]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (113.14,364) -- (120.65,364) -- (120.65,357) -- (113.14,357) -- cycle ;
%Shape: Rectangle [id:dp9003849208574134]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (120.65,364) -- (128.17,364) -- (128.17,357) -- (120.65,357) -- cycle ;
%Shape: Rectangle [id:dp5853979347141709]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (173.99,366.15) -- (233.65,366.15) -- (233.65,386) -- (173.99,386) -- cycle ;
%Shape: Rectangle [id:dp621024419525601]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (172.99,420.33) -- (232.65,420.33) -- (232.65,439.33) -- (172.99,439.33) -- cycle ;
%Straight Lines [id:da33216483634168326]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (235.65,379.68) -- (256.49,379.77) ;
\draw [shift={(232.65,379.67)}, rotate = 0.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da9112661943078489]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (234.65,429.68) -- (258.49,429.77) ;
\draw [shift={(231.65,429.67)}, rotate = 0.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da9399093259342111]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (236.65,348.71) -- (257.11,349.03) ;
\draw [shift={(233.65,348.67)}, rotate = 0.9] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da043622843220090024]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (360.49,388) -- (380.49,388) ;
\draw [shift={(357.49,388)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%%astuce

% aumenter premier pour decaler a droite, dinuer pour decaler à gauche.
% agmeter second pour decendre en bas, diminuer pour monter en haut
% Text Node
\draw (141.7,355.73) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-88.73] [align=center] {Message concatenation};
% Text Node
\draw (319.82,381.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {De-Rate \\Matching};
% Text Node
\draw (382.99,383.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {De-Modulation};
% Text Node
\draw (453.99,379.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=center] {Resource\\Extraction};
% Text Node
\draw (504.99,376.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$y$};
% Text Node
\draw (78.65,356.8) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.15]  {$\cdots $};
% Text Node
\draw (31.76,343) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {$K$- recovered message bits};
% Text Node
\draw (13,362.01) node [anchor=north west][inner sep=0.5pt]  [font=\tiny,xslant=-0.0004]  {$\ \ \ \ \ \underbrace{\ \ \ \ \ \ \ \ \ \ \ \ \ }_{\hat{\bm B}{^{( 1)}}}$};
% Text Node
\draw (41.74,362.01) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,xslant=-0.04]  {$\ \ \ \ \ \underbrace{\ \ \ \ \ \ \ \ \ \ \ }_{\hat{\bm B}{^{( 2)}}}$};
% Text Node
\draw (180.99,347.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] { HT/FHT Dec.};
% Text Node
\draw (278.16,354.1) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-88.73] [align=left] {CB \ De-Concatenation\\+ \ Bipolar Mapping \ };
% Text Node
\draw (180.99,339.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$^{(1)}$};
% Text Node
\draw (80.74,362.01) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,xslant=-0.04]  {$\ \ \ \ \ \underbrace{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }_{\hat{\bm B}{^{(\mathcal N)}}}$};
% Text Node
\draw (180.99,376.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] { HT/FHT Dec.};
% Text Node
\draw (194.99,386.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (180.99,367.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$^{(2)}$};
% Text Node
\draw (180.99,429.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] { HT/FHT Dec.};
% Text Node
\draw (180.99,421.73) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$^{(\mathcal N)}$};
% Text Node
\draw (248.99,341.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {};


\end{tikzpicture}


==> figures/tikzfigure/tx_propose.tex <==


\tikzset{every picture/.style={line width=0.25pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,672); %set diagram left start at 0, and has height of 672

%Shape: Rectangle [id:dp534691631513805]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (28,61.15) -- (37.8,61.15) -- (37.8,68.07) -- (28,68.07) -- cycle ;
%Shape: Rectangle [id:dp14817412932548069]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (135,41) -- (147.12,41) -- (147.12,143.03) -- (135,143.03) -- cycle ;
%Shape: Rectangle [id:dp6472264046042663]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (298.83,79.15) -- (343.33,79.15) -- (343.33,101.67) -- (298.83,101.67) -- cycle ;
%Shape: Rectangle [id:dp8157514209446664]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (366,80.15) -- (412.83,80.15) -- (412.83,100.67) -- (366,100.67) -- cycle ;
%Shape: Rectangle [id:dp6754040384549601]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (434,79.67) -- (475.33,79.67) -- (475.33,100.67) -- (434,100.67) -- cycle ;
%Straight Lines [id:da03369569056376753]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (31.67,86.67) -- (130.25,86.19) ;
\draw [shift={(133.25,86.17)}, rotate = 179.72] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da7640143617506934]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (271,89) -- (296.25,89.16) ;
\draw [shift={(299.25,89.17)}, rotate = 180.35] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da9298206759216789]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (411.5,90) -- (431.5,90) ;
\draw [shift={(434.5,90)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da8045824119808925]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (474.5,90) -- (491.5,90) ;
\draw [shift={(494.5,90)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Shape: Rectangle [id:dp8058948611223219]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (177,42.15) -- (236.67,42.15) -- (236.67,62) -- (177,62) -- cycle ;
%Shape: Rectangle [id:dp02162926917450747]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (37.8,61.15) -- (47.61,61.15) -- (47.61,68.07) -- (37.8,68.07) -- cycle ;
%Shape: Rectangle [id:dp22728084022677342]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (47.61,61.15) -- (57.41,61.15) -- (57.41,68.07) -- (47.61,68.07) -- cycle ;
%Shape: Rectangle [id:dp04815469931187599]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (57.41,61.07) -- (66.78,61.07) -- (66.78,68.07) -- (57.41,68.07) -- cycle ;
%Shape: Rectangle [id:dp9126821467798913]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (66.78,61.07) -- (76.15,61.07) -- (76.15,68.07) -- (66.78,68.07) -- cycle ;
%Shape: Rectangle [id:dp7508084829627262]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (76.15,68) -- (83.67,68) -- (83.67,61) -- (76.15,61) -- cycle ;
%Straight Lines [id:da21335610677557737]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (146.67,47.67) -- (174,48.1) ;
\draw [shift={(177,48.15)}, rotate = 180.91] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da873056744522289]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (147.67,82.67) -- (175.67,82.67) ;
\draw [shift={(178.67,82.67)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da8265803661513512]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (146.67,130.67) -- (172.67,130.67) ;
\draw [shift={(175.67,130.67)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Shape: Rectangle [id:dp10012600562072582]
\draw  [fill={rgb, 255:red, 32; green, 142; blue, 189 }  ,fill opacity=1 ] (260,43.03) -- (270.12,43.03) -- (270.12,146.03) -- (260,146.03) -- cycle ;
%Shape: Rectangle [id:dp5779827634553952]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (97.41,61.07) -- (106.78,61.07) -- (106.78,68.07) -- (97.41,68.07) -- cycle ;
%Shape: Rectangle [id:dp9677885115632103]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (106.78,61.07) -- (116.15,61.07) -- (116.15,68.07) -- (106.78,68.07) -- cycle ;
%Shape: Rectangle [id:dp27830143247872696]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (116.15,68) -- (123.67,68) -- (123.67,61) -- (116.15,61) -- cycle ;
%Shape: Rectangle [id:dp8104799095076661]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (123.67,68) -- (131.18,68) -- (131.18,61) -- (123.67,61) -- cycle ;
%Shape: Rectangle [id:dp5830181859019739]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 185 }  ,fill opacity=1 ] (177,70.15) -- (236.67,70.15) -- (236.67,90) -- (177,90) -- cycle ;
%Shape: Rectangle [id:dp3248509231261022]
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (176,124.33) -- (235.67,124.33) -- (235.67,143.33) -- (176,143.33) -- cycle ;
%Straight Lines [id:da9914106204618699]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (236.67,80.67) -- (257.5,80.76) ;
\draw [shift={(260.5,80.77)}, rotate = 180.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da039899876527087264]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (235.67,132.67) -- (259.5,132.76) ;
\draw [shift={(262.5,132.77)}, rotate = 180.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da6715929168334498]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (236.67,52.67) -- (257.13,52.99) ;
\draw [shift={(260.12,53.03)}, rotate = 180.9] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;
%Straight Lines [id:da4876065562975156]
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (343.5,90) -- (363.5,90) ;
\draw [shift={(366.5,90)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- (3.56,0) -- cycle    ;

% Text Node
\draw (143.71,53.73) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-88.73] [align=left] {Message Segmentation};
% Text Node
\draw (304.88,82.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=center] { \ \ \ \ Rate \\Matching};
% Text Node
\draw (371,86.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=center] {Modulation};
% Text Node
\draw (440,83.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=center] {Resource\\ Mapping};
% Text Node
\draw (489,81.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$N=N_d+N_p$};
% Text Node
\draw (81.66,60.41) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.15]  {$\cdots $};
% Text Node
\draw (58.77,45) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {$K$-message bits};
% Text Node
\draw (15.15,65.01) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,xslant=-0.04]  {$\ \ \ \ \ \underbrace{\ \ \ \ \ \ \  \ \ \ \ \ \ }_{\bm B{^{(1)}}}$};
% Text Node
\draw (44.75,65.01) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,xslant=-0.04]  {$\ \ \ \ \ \underbrace{\ \ \ \ \ \ \ \ \ \ \ }_{\bm B{^{(2)}}}$};
% Text Node
\draw (188,51.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] { RM(1, m) Enc.};
% Text Node
\draw (267.17,51.1) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-88.73] [align=left] {Code block \ Concatenation};
% Text Node
\draw (188,43.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$^{(1)}$};
% Text Node
\draw (83.75,65.01) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,xslant=-0.04]  {$\ \ \ \ \ \underbrace{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }_{\bm B{^{(\mathcal N)}}}$};
% Text Node
\draw (188,80.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] { RM(1, m) Enc.};
% Text Node
\draw (198,88.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots$};
% Text Node
\draw (188,71.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$^{(2)}$};
% Text Node
\draw (188.67,133.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {RM(1, m) Enc.};
% Text Node
\draw (188,125.73) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$^{(\mathcal N)}$};


\end{tikzpicture}

